FLAME: Towards Federated Fine-Tuning Large Language Models Through Adaptive SMoE

Existing resource-adaptive LoRA federated fine-tuning methods enable clients to fine-tune models using compressed versions of global LoRA matrices, in order to accommodate various compute resources across clients. This compression requirement will lead to suboptimal performance due to information loss. To address this, we propose FLAME, a novel federated learning framework based on the Sparse Mixture-of-Experts (SMoE) architecture. Unlike prior approaches, FLAME retains full (uncompressed) global LoRA matrices and achieves client-side adaptability by varying the number of activated experts per client. However, incorporating SMoE into federated learning introduces unique challenges, specifically, the mismatch in output magnitude from partial expert activation and the imbalance in expert training quality across clients. FLAME tackles these challenges through a lightweight rescaling mechanism and an activation-aware aggregation scheme. Empirical results across diverse computational settings demonstrate that FLAME consistently outperforms existing methods, providing a robust and effective solution for resource-adaptive federated learning.

==> sections/intro.tex <==
\section{Introduction}

%background: 1. Large Language Models is successful; 2. Large Language Models need to be fine-tuned; 3. collecting such datasets raises concerns about cost and privacy; 4. because of 3 we need Federated Learning; 5. in the field of 4 LoRA become attractive.
Large language models (LLMs) have achieved remarkable success across a wide range of tasks, largely due to extensive pre-training on massive datasets  \cite{achiam2023gpt, dong2023towards, kelly2023bing, thirunavukarasu2023large}. While these models demonstrate impressive capabilities, fine-tuning remains essential to adapt them for specific applications and domains \cite{parthasarathy2024ultimate, anisuzzaman2025fine}. 
However, centralizing sensitive data for fine-tuning raises significant privacy concerns \cite{voigt2017eu, pardau2018california}, making traditional fine-tuning approaches increasingly problematic.
Federated Learning (FL), therefore, has emerged as a promising solution that enables model improvement while keeping data decentralized \cite{zhang-etal-2023-fedpet, kuang2024federatedscope, woisetschlager2024federated, wu2025survey}. Within this framework, parameter-efficient fine-tuning techniques—particularly Low-Rank Adaptation (LoRA)—have gained much attention due to their ability to effectively adapt models with minimal computational overhead \cite{hu2022, ding2023parameter}. 

%brief intro about current methods 
In federated learning, a fundamental challenge is balancing the heterogeneity of resources across clients. Existing approaches \cite{cho-etal-2024-heterogeneous,bai2024federated}  typically maintain global LoRA matrices on central servers, while requiring each client to use a compressed version of the global LoRA matrices that aligns with its own computational constraints—typically by reducing the rank.  
%and their drawbacks
These methods balance heterogeneous client capabilities primarily through matrix decomposition, particularly Singular Value Decomposition (SVD), operating under the assumption that higher-rank matrices preserve more information. 
Such a design deals with heterogeneity by allowing resource-constrained clients to use lower-rank approximations of the global LoRA matrices, while resource-rich clients can utilize higher-rank representations. 
Research has demonstrated that the importance ranking of singular values from SVD does not always align optimally with preserving LLM performance on downstream tasks \cite{hsulanguage,hua2022numerical}. 
Furthermore, this matrix decomposition-based strategy has inherent limitations: the diversity in local clients is achieved through the compression of global LoRA matrices at different levels. That is to say, in order to accommodate diverse client capabilities, all local models are inherently forced to discard part of the knowledge encoded in the global LoRA matrices, which is obviously suboptimal \ting{any citation}. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figs/Flame.pdf}
    \caption{An illustration of resource-adaptive federated fine-tuning with \modelname. }
    \label{fig-FLAME}
\end{figure}

Building on this idea, we propose a novel method called \modelname. As illustrated in Figure~\ref{fig-FLAME}, \modelname{} leverages the SMoE architecture to enable each client to fine-tune the model using full (uncompressed) global LoRA matrices. The number of activated experts varies across clients based on their compute capacity (e.g., client $c_1$ activates more experts than client $c_3$), allowing resource-adaptive fine-tuning without structural compression.

However, this design presents two key challenges. First, partial expert activation leads to a mismatch in output magnitude compared to full-capacity execution. To address this, \modelname{} introduces a lightweight rescaling module that realigns expert outputs across clients. Second, variations in client-specific training quality result in inconsistencies in expert LoRA matrices, which can compromise the global aggregation. To solve this problem, \modelname{} incorporates an activation-aware aggregation scheme that weights each expert's contribution based on its activation pattern during training.
Our contributions can be summarized as follows:

\begin{itemize}
\item \textbf{Resource-Adaptive Sparse Expert Selection}: We introduce \modelname, a novel federated learning framework that leverages sparse mixture-of-experts (SMoE) architecture to enable resource-adaptive fine-tuning without compromising the expressive power of global LoRA matrices. Unlike existing compression-based approaches, our method maintains full global LoRA matrices while varying the number of activated experts according to client computational capabilities.
\item \textbf{Output alignment through lightweight rescaling}: We develop a lightweight learnable rescaling mechanism that adaptively calibrates the output magnitude of partially activated expert layers, effectively compensating for the reduced expert participation while preserving model performance. This approach is more flexible than static rescaling and accounts for the dynamic nature of SMoE activations.
\item \textbf{Activation-aware aggregation}:  We identify and address the critical issue of imbalanced expert training across heterogeneous clients by proposing an activation-aware aggregation scheme. This scheme dynamically adjusts the contribution of each expert based on its activation frequencies, ensuring consistent global LoRA matrix synthesis across clients. Empirical evaluations demonstrate that our approach consistently outperforms existing resource-adaptive federated fine-tuning methods across various computational settings.
\end{itemize}
